ACD-GS: Asymmetric Curvature-aware Densification for 3D Gaussian Splatting

3D Gaussian Splatting (3DGS) has emerged as a powerful paradigm for real-time photorealistic novel view synthesis. However, its training-time densification remains largely heuristic, often resulting in redundant Gaussian proliferation and inaccurate geometric reconstruction. Existing methods predominantly rely on first-order screen-space gradients to trigger cloning and splitting, which fail to distinguish true geometric discontinuities from high-frequency textures or noisy residuals. To address this limitation, we propose ACD-GS, an Asymmetric Curvature-aware Densification framework for compact and geometry-aware 3D Gaussian optimization. Our key insight is that second-order depth responses provide a more reliable structural prior for density control, enabling asymmetric regulation of cloning and splitting to better capture geometric discontinuities. Building on this, we introduce a multi-view photometric consistency constraint to suppress transient single-view errors, together with a capacity-aware adaptive regulation strategy that balances densification and pruning during training. Unlike post-hoc compression or quantization-based approaches, ACD-GS directly prevents redundant Gaussian generation during training, yielding inherently compact representations. Extensive experiments demonstrate that our method reduces nearly 60% of Gaussian count and storage while maintaining competitive rendering fidelity, consistently outperforming existing methods across multiple datasets. Our code is available in https://waveviewer.github.io/ACD-GS/.

==> tables/alpha_beta_v8.tex <==
\begin{table}[t]
  \centering
  \caption{Comparison of different settings for $\alpha$ and $\beta$, varying one parameter at a time.}
  \label{tab:parametre10}
  \small
  \begin{tabular}{@{}cccccc@{}}
    \toprule
    $\alpha$ & $\beta$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & Size(MB)$\downarrow$ \\
    \midrule
0.5 & 1.5 & 25.5890 & 0.8424 & 0.2387 & 161.37\\
0.8 & 1.5 & 25.5913 & 0.8450 & \textbf{0.2363} & \textbf{151.85}\\
1.0 & 1.5 & \textbf{25.8259} & \textbf{0.8469} & 0.2520 & 162.54\\
\midrule
0.8 & 1.0 & 25.4263 & 0.8412 & 0.2451 & 157.35\\
0.8 & 2.5 & 25.4441 & 0.8415 & 0.2436 & 164.87\\
    \bottomrule
  \end{tabular}
\end{table}

